CodeTailor: LLM-Powered Personalized Parsons Puzzles for Engaging Support While Learning Programming

Learning to program can be challenging, and providing high-quality and timely support at scale is hard. Generative AI and its products, like ChatGPT, can create a solution for most intro-level programming problems. However, students might use these tools to just generate code for them, resulting in reduced engagement and limited learning. In this paper, we present CodeTailor, a system that leverages a large language model (LLM) to provide personalized help to students while still encouraging cognitive engagement. CodeTailor provides a personalized Parsons puzzle to support struggling students. In a Parsons puzzle, students place mixed-up code blocks in the correct order to solve a problem. A technical evaluation with previous incorrect student code snippets demonstrated that CodeTailor could deliver high-quality (correct, personalized, and concise) Parsons puzzles based on their incorrect code. We conducted a within-subjects study with 18 novice programmers. Participants perceived CodeTailor as more engaging than just receiving an LLM-generated solution (the baseline condition). In addition, participants applied more supported elements from the scaffolded practice to the posttest when using CodeTailor than baseline. Overall, most participants preferred using CodeTailor versus just receiving the LLM-generated code for learning. Qualitative observations and interviews also provided evidence for the benefits of CodeTailor, including thinking more about solution construction, fostering continuity in learning, promoting reflection, and boosting confidence. We suggest future design ideas to facilitate active learning opportunities with generative AI techniques.

==> Sections/7_conclusion.tex <==
\section{Conclusion}
We created \sys{}, a novel system to provide active and two-staged personalized scaffolding for students while writing code. \sys{} provides two-staged personalized Parsons puzzles that include correct solutions based on students' incorrect code, as well as pre-placement of correct lines. Additionally, student erroneous lines are reused as distractors, and movable lines can be conditionally combined. The technical evaluation demonstrated that \sys{} can reliably generate high-quality Parsons puzzles with solutions similar to the student's existing code state and can be solved more effectively than conventional fully movable Parsons puzzles. The student evaluation shows that \sys{} was more engaging to use, and students were able to use more help-derived components to solve the posttest after using \sys{} instead of just getting the right answer, which is the normal LLM output. Additionally, students preferred \sys{} for the sake of learning over the normal LLM output. This work illustrates how we can reduce over-reliance on learning with LLM by providing real-time active help during problem-solving.
